CollabCoder: A Lower-barrier, Rigorous Workflow for Inductive Collaborative Qualitative Analysis with Large Language Models

Collaborative Qualitative Analysis (CQA) can enhance qualitative analysis rigor and depth by incorporating varied viewpoints. Nevertheless, ensuring a rigorous CQA procedure itself can be both demanding and costly. To lower this bar, we take a theoretical perspective to design the CollabCoder workflow, that integrates Large Language Models (LLMs) into key inductive CQA stages: independent open coding, iterative discussions, and final codebook creation. In the open coding phase, CollabCoder offers AI-generated code suggestions and records decision-making data. During discussions, it promotes mutual understanding by sharing this data within the coding team and using quantitative metrics to identify coding (dis)agreements, aiding in consensus-building. In the code grouping stage, CollabCoder provides primary code group suggestions, lightening the cognitive load of finalizing the codebook. A 16-user evaluation confirmed the effectiveness of CollabCoder, demonstrating its advantages over existing software and providing empirical insights into the role of LLMs in the CQA practice.

==> paper/5_results_old.tex <==
\section{Results}

\added{\textbf{RQ2. How does CollabCoder compare to currently available tools like Atlas.ti Web?}}

\subsection{Quantitative Results}

\begin{table*}[!t]
\caption{Overview of the final coding results. "Collab." denotes \diffcoder, "Atlas." denotes Atlas.ti Web, "Total Codes" denotes the total number of codes generated while "Discussed Codes" denotes the total number of codes that were discussed by the coders during the discussion phase. "Bus." denotes the "Business" dataset while "His." denotes the "History" dataset.}
\label{tab:result}
\scalebox{0.55}{
\begin{tabular}{|cccc|cc|cc|cc|cc|cc|cc|c|c|}
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{\textbf{Pairs}}} & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Self-reported\\ QA expertise\end{tabular}}}} & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Conditions}}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Collaboration\\ Observation\end{tabular}}} & \multicolumn{2}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Total Codes\end{tabular}}} & \multicolumn{2}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Discussed\\ Codes (No.)\end{tabular}}} & \multicolumn{2}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}IRR (-1 to 1)\end{tabular}}} & \multicolumn{2}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Code Groups (No.)\end{tabular}}} & \multicolumn{2}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Discussion \\ Time (mins:secs)\end{tabular}}} & \multicolumn{2}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}\small{Open Codes} \\[-0.4em] \small{Sources (\%)}\end{tabular}}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Self-proposed\\ Codes (\%)\end{tabular}}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Final \\ Codes \\ Sources (\%)\end{tabular}}} \\ \cline{5-16}
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} &  & \multicolumn{1}{c|}{\textbf{Collab.}} & \textbf{Atlas.} & \multicolumn{1}{c|}{\textbf{Collab.}} & \textbf{Atlas.} & \multicolumn{1}{c|}{\textbf{Collab.\textsuperscript{b}}} & \textbf{Atlas.} & \multicolumn{1}{c|}{\textbf{Collab.}} & \textbf{Atlas.} & \multicolumn{1}{c|}{\textbf{Collab.}} & \textbf{Atlas.} & \multicolumn{1}{c|}{\textbf{GPT}} & \textbf{Rele.} &  &  \\ \hline
\multicolumn{1}{|c|}{P1} & \multicolumn{1}{c|}{Beginner} & \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Atlas. (Bus.), \\ Collab.His.)\end{tabular}}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Follower-\\ Leader\end{tabular}} & \multicolumn{1}{c|}{\multirow{2}{*}{15}} & \multirow{2}{*}{24} & \multicolumn{1}{c|}{\multirow{2}{*}{15}} & \multirow{2}{*}{6} & \multicolumn{1}{c|}{\multirow{2}{*}{NA}} & \multirow{2}{*}{-0.07} & \multicolumn{1}{c|}{\multirow{2}{*}{6}} & \multirow{2}{*}{3} & \multicolumn{1}{c|}{\multirow{2}{*}{19:41}} & \multirow{2}{*}{07:39} & \multicolumn{1}{c|}{100} & 0 & 0 & \multirow{2}{*}{5} \\ \cline{15-17}
\multicolumn{1}{|c|}{P2} & \multicolumn{1}{c|}{No Experience} & \multicolumn{1}{c|}{} &  & \multicolumn{1}{c|}{} &  & \multicolumn{1}{c|}{} &  & \multicolumn{1}{c|}{} &  & \multicolumn{1}{c|}{} &  & \multicolumn{1}{c|}{} &  & \multicolumn{1}{c|}{70} & 5 & 25 &  \\ \hline
\multicolumn{1}{|c|}{P3} & \multicolumn{1}{c|}{Expert} & \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Collab.(Bus.), \\ Atlas. (His.)\end{tabular}}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Amicable \\ Cooperation\end{tabular}} & \multicolumn{1}{c|}{\multirow{2}{*}{15}} & \multirow{2}{*}{10} & \multicolumn{1}{c|}{\multirow{2}{*}{15}} & \multirow{2}{*}{10} & \multicolumn{1}{c|}{\multirow{2}{*}{NA}} & \multirow{2}{*}{1} & \multicolumn{1}{c|}{\multirow{2}{*}{5}} & \multirow{2}{*}{4} & \multicolumn{1}{c|}{\multirow{2}{*}{35:24}} & \multirow{2}{*}{21:32} & \multicolumn{1}{c|}{90} & 0 & 10 & \multirow{2}{*}{40} \\ \cline{15-17}
\multicolumn{1}{|c|}{P4} & \multicolumn{1}{c|}{No Experience} & \multicolumn{1}{c|}{} &  & \multicolumn{1}{c|}{} &  & \multicolumn{1}{c|}{} &  & \multicolumn{1}{c|}{} &  & \multicolumn{1}{c|}{} &  & \multicolumn{1}{c|}{} &  & \multicolumn{1}{c|}{90} & 0 & 10 &  \\ \hline
\multicolumn{1}{|c|}{P5} & \multicolumn{1}{c|}{No Experience} & \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Atlas. (His.), \\ Collab.(Bus.)\end{tabular}}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Follower-\\ Leader\end{tabular}} & \multicolumn{1}{c|}{\multirow{2}{*}{15}} & \multirow{2}{*}{11} & \multicolumn{1}{c|}{\multirow{2}{*}{15}} & \multirow{2}{*}{2} & \multicolumn{1}{c|}{\multirow{2}{*}{NA}} & \multirow{2}{*}{-0.02} & \multicolumn{1}{c|}{\multirow{2}{*}{5}} & \multirow{2}{*}{2} & \multicolumn{1}{c|}{\multirow{2}{*}{17:55}} & \multirow{2}{*}{06:16} & \multicolumn{1}{c|}{73} & 7 & 20 & \multirow{2}{*}{100} \\ \cline{15-17}
\multicolumn{1}{|c|}{P6} & \multicolumn{1}{c|}{Expert} & \multicolumn{1}{c|}{} &  & \multicolumn{1}{c|}{} &  & \multicolumn{1}{c|}{} &  & \multicolumn{1}{c|}{} &  & \multicolumn{1}{c|}{} &  & \multicolumn{1}{c|}{} &  & \multicolumn{1}{c|}{100} & 0 & 0 &  \\ \hline
\multicolumn{1}{|c|}{P7} & \multicolumn{1}{c|}{No Experience} & \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Collab.(His.)\\ Atlas. (Bus.)\end{tabular}}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Amicable \\ Cooperation\end{tabular}} & \multicolumn{1}{c|}{\multirow{2}{*}{15}} & \multirow{2}{*}{22} & \multicolumn{1}{c|}{\multirow{2}{*}{15}} & \multirow{2}{*}{2} & \multicolumn{1}{c|}{\multirow{2}{*}{NA}} & \multirow{2}{*}{-0.33} & \multicolumn{1}{c|}{\multirow{2}{*}{7}} & \multirow{2}{*}{6} & \multicolumn{1}{c|}{\multirow{2}{*}{29:08}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}No \\ discussion\textsuperscript{a}\end{tabular}} & \multicolumn{1}{c|}{7} & 0 & 93 & \multirow{2}{*}{80} \\ \cline{15-17}
\multicolumn{1}{|c|}{P8} & \multicolumn{1}{c|}{No Experience} & \multicolumn{1}{c|}{} &  & \multicolumn{1}{c|}{} &  & \multicolumn{1}{c|}{} &  & \multicolumn{1}{c|}{} &  & \multicolumn{1}{c|}{} &  & \multicolumn{1}{c|}{} &  & \multicolumn{1}{c|}{13} & 7 & 80 &  \\ \hline
\multicolumn{1}{|c|}{P9} & \multicolumn{1}{c|}{Intermediate} & \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Atlas. (Bus.), \\ Collab.(His.)\end{tabular}}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Amicable \\ Cooperation\end{tabular}} & \multicolumn{1}{c|}{\multirow{2}{*}{15}} & \multirow{2}{*}{17} & \multicolumn{1}{c|}{\multirow{2}{*}{15}} & \multirow{2}{*}{5} & \multicolumn{1}{c|}{\multirow{2}{*}{NA}} & \multirow{2}{*}{0.04} & \multicolumn{1}{c|}{\multirow{2}{*}{5}} & \multirow{2}{*}{2} & \multicolumn{1}{c|}{\multirow{2}{*}{15:11}} & \multirow{2}{*}{14:38} & \multicolumn{1}{c|}{73} & 13 & 13 & \multirow{2}{*}{80} \\ \cline{15-17}
\multicolumn{1}{|c|}{P10} & \multicolumn{1}{c|}{No Experience} & \multicolumn{1}{c|}{} &  & \multicolumn{1}{c|}{} &  & \multicolumn{1}{c|}{} &  & \multicolumn{1}{c|}{} &  & \multicolumn{1}{c|}{} &  & \multicolumn{1}{c|}{} &  & \multicolumn{1}{c|}{53} & 40 & 7 &  \\ \hline
\multicolumn{1}{|c|}{P11} & \multicolumn{1}{c|}{Intermediate} & \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Collab.(Bus.), \\ Atlas. (His.)\end{tabular}}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Quick and\\ not careful\end{tabular}} & \multicolumn{1}{c|}{\multirow{2}{*}{15}} & \multirow{2}{*}{61} & \multicolumn{1}{c|}{\multirow{2}{*}{15}} & \multirow{2}{*}{2} & \multicolumn{1}{c|}{\multirow{2}{*}{NA}} & \multirow{2}{*}{-0.07} & \multicolumn{1}{c|}{\multirow{2}{*}{3}} & \multirow{2}{*}{3} & \multicolumn{1}{c|}{\multirow{2}{*}{19:23}} & \multirow{2}{*}{14:15} & \multicolumn{1}{c|}{100} & 0 & 0 & \multirow{2}{*}{100} \\ \cline{15-17}
\multicolumn{1}{|c|}{P12} & \multicolumn{1}{c|}{No experience} & \multicolumn{1}{c|}{} &  & \multicolumn{1}{c|}{} &  & \multicolumn{1}{c|}{} &  & \multicolumn{1}{c|}{} &  & \multicolumn{1}{c|}{} &  & \multicolumn{1}{c|}{} &  & \multicolumn{1}{c|}{100} & 0 & 0 &  \\ \hline
\multicolumn{1}{|c|}{P13} & \multicolumn{1}{c|}{Beginner} & \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Atlas. (His.), \\ Collab.(Bus.)\end{tabular}}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Amicable \\ Cooperation\end{tabular}} & \multicolumn{1}{c|}{\multirow{2}{*}{15}} & \multirow{2}{*}{30} & \multicolumn{1}{c|}{\multirow{2}{*}{15}} & \multirow{2}{*}{5} & \multicolumn{1}{c|}{\multirow{2}{*}{NA}} & \multirow{2}{*}{-0.08} & \multicolumn{1}{c|}{\multirow{2}{*}{8}} & \multirow{2}{*}{2} & \multicolumn{1}{c|}{\multirow{2}{*}{29:19}} & \multirow{2}{*}{08:43} & \multicolumn{1}{c|}{87} & 7 & 7 & \multirow{2}{*}{100} \\ \cline{15-17}
\multicolumn{1}{|c|}{P14} & \multicolumn{1}{c|}{Intermediate} & \multicolumn{1}{c|}{} &  & \multicolumn{1}{c|}{} &  & \multicolumn{1}{c|}{} &  & \multicolumn{1}{c|}{} &  & \multicolumn{1}{c|}{} &  & \multicolumn{1}{c|}{} &  & \multicolumn{1}{c|}{93} & 0 & 7 &  \\ \hline
\multicolumn{1}{|c|}{P15} & \multicolumn{1}{c|}{Beginner} & \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Collab.(His.)\\ Atlas. (Bus.)\end{tabular}}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Amicable \\ Cooperation\end{tabular}} & \multicolumn{1}{c|}{\multirow{2}{*}{15}} & \multirow{2}{*}{8} & \multicolumn{1}{c|}{\multirow{2}{*}{15}} & \multirow{2}{*}{4} & \multicolumn{1}{c|}{\multirow{2}{*}{NA}} & \multirow{2}{*}{0.04} & \multicolumn{1}{c|}{\multirow{2}{*}{4}} & \multirow{2}{*}{2} & \multicolumn{1}{c|}{\multirow{2}{*}{29:09}} & \multirow{2}{*}{08:52} & \multicolumn{1}{c|}{100} & 0 & 0 & \multirow{2}{*}{43} \\ \cline{15-17}
\multicolumn{1}{|c|}{P16} & \multicolumn{1}{c|}{No experience} & \multicolumn{1}{c|}{} &  & \multicolumn{1}{c|}{} &  & \multicolumn{1}{c|}{} &  & \multicolumn{1}{c|}{} &  & \multicolumn{1}{c|}{} &  & \multicolumn{1}{c|}{} &  & \multicolumn{1}{c|}{73} & 20 & 7 &  \\ \hline
\multicolumn{4}{|c|}{Mean} & \multicolumn{1}{c|}{15} & 22.88 & \multicolumn{1}{c|}{15} & 4.5 & \multicolumn{1}{c|}{NA} & 0.06 & \multicolumn{1}{c|}{5.38} & 3 & \multicolumn{1}{c|}{24:00} & 10:48 & \multicolumn{1}{c|}{76.46} & 6.15 & 17.4 & 68.5 \\ \hline
\multicolumn{4}{|c|}{SD} & \multicolumn{1}{c|}{0} & 17.19 & \multicolumn{1}{c|}{0} & 2.73 & \multicolumn{1}{c|}{NA} & 0.40 & \multicolumn{1}{c|}{1.60} & 1.41 & \multicolumn{1}{c|}{07:12} & 05:24 & \multicolumn{1}{c|}{29.43} & 10.74 & 28.11 & 35.3 \\ \hline
\end{tabular}
}

\vspace{1ex}
\raggedright
\footnotesize
\textsuperscript{a} P7 and P8 gave up discussion for the Atlas.ti session due to spending too much time in the \diffcoder session. \\
\textsuperscript{b} Following the discussion session in \diffcoder, the original codes have been restructured and finalized as a single code decision, resulting in an IRR$\approx$1. Consequently, IRR calculations are not applicable for the \diffcoder conditions. 

\end{table*}



\subsubsection{Post-study questionnaire}

We gathered the subjective preferences from our participants. To do so, we gave them 12 statements like \textit{"I find it effective to..."} and \textit{"I feel confident/prefer..."} pertaining to the effectiveness and self-perception. We then asked them to rate their agreement with each sentence on a 5-point Likert scale for each platform. The details of the 12 statements are shown in Figure~\ref{fig:results}.

Overall, pairwise t-tests showed that participants rated \diffcoder significantly (all $p<.05$) better than Atlas.ti Web for effectiveness in 1) \textit{coming up with codes}, 2) \textit{producing final code groups}, 3) \textit{identifying disagreements}, 4) \textit{resolving disagreements and making decisions}, 5) \textit{understanding the current level of agreement}, and 6) \textit{understanding others' thoughts}. The results also indicated that participants believed \diffcoder could be learned for use quickly compared to Atlas.ti Web ($t(15) = -3.05, p < .01$).
For other dimensions, the \textit{confidence in the final quality}, \textit{perceived level of preference}, \textit{level of control}, \textit{level of understanding}, and \textit{ease of use}, while our results show a general trend where \diffcoder achieves higher scores, we found no significant differences. 
Additionally, we observed that one expert user (P6) exhibited a highly negative attitude towards implementing AI in qualitative coding, as he selected "strongly disagree" for nearly all assessment criteria. We will discuss his qualitative feedback later. 


\subsubsection{Log Data Analysis}
A two-tailed pairwise t-test on \textit{Discussion Time} revealed a significant difference ($t(15) = -3.22, p = .017$) between \diffcoder $(M\approx24mins, SD\approx7mins)$ and Atlas.ti Web $(M\approx11mins, SD\approx5.5mins)$. \textbf{Discussions under the \diffcoder condition were significantly longer than those in the Atlas.ti Web condition.}
When examining the IRR, it was found that the IRRs in the Atlas.ti Web condition were overall significantly ($t(7)=-6.69, p<.001$) lower $(M=0.06, SD =0.40)$, compared to the \diffcoder condition ($M \approx 1$).
In the latter, participants thoroughly examined all codes, resolved conflicts, merged similar codes, and reached a final decision for each data unit.
Conversely, Atlas.ti Web posed challenges in comparing individual data units side-by-side, leading to minimal code discussions overall (averaging 4.5 codes discussed) compared to the \diffcoder option (averaging 15 codes discussed). Consequently, we surmise that concealed disagreements within Atlas.ti Web might require additional discussion rounds to attain a higher agreement level. Further evidence is needed to validate this assumption.


\subsection{Qualitative Results}
\subsubsection{Data analysis}
We analyzed interview transcripts and observation notes (see Table \ref{tab:observation_notes_1} and \ref{tab:observation_notes_2}) using thematic analysis as described in Braun and Clarke’s methodology~\cite{braun2006using}. After familiarizing ourselves with data and generating initial codes, we grouped the transcripts into common themes based on the content. Next, we discussed, interpreted, and resolved discrepancies or conflicts during the grouping process. Finally, we reviewed the transcripts to extract specific quotes relevant to each theme. We summarized the following key findings.


\subsubsection{Key Findings (KF) on Features}

\added{\\\textbf{RQ1: Can CollabCoder support qualitative coders conduct CQA effectively?}}

\paragraph{KF1: \textit{\diffcoder} workflow simplifies the learning curve for CQA and ensures coding independence in the initial stages.}
\label{sec:results:KF1}

Overall, users found \diffcoder to be better as it supports side-by-side comparison of data, which makes coding and discussion process \textbf{easier to understand (P2), more straightforward (P7), and beginner-friendly (P4)} than Atlas.ti Web, and P4 noted that \diffcoder had a \textbf{lower learning curve}.


Moreover, \diffcoder workflow preserves coding independence. Experienced users (P11 and P14), familiar with qualitative analysis, find \textit{\diffcoder}'s independent coding feature to be particularly beneficial: \textit{"So you don't see what the other person is coding until like both of you are done. So it doesn't like to affect your own individual coding...[For Atlas.ti Web] the fact like you can see both persons’ codes and I think I'm able to edit the other person's codes as well, which I think might not be very a good practice."}
Similarly, P14 indicated: \textit{"I think \diffcoder is better if you aim for independent coding."}


\paragraph{KF2: Individual workspace with GPT assistance is valued for reducing cognitive burden.}
\label{sec:results:KF2}

\diffcoder makes it easier for beginner users to propose and edit codes compared to Atlas.ti Web. 7/16 participants appreciated that GPT's additional assistance (P7, P15), which gave them reference (P1) and decreased thinking (P9). Such feelings are predominantly reported by individuals who are either beginners or lack prior experience in qualitative analysis.
As P13 said, \textit{"I think the \diffcoder one is definitely more intuitive in a sense, because it provides some suggestion, you might not use it, but at least some basic suggestions, whereas the Atlas.ti one, you have to take from scratch and it takes more mental load."} (P13). 


Some of these beginners also showed displeasure towards GPT, largely stems from its content summarization level, which users cannot regulate. 
P1 (beginner) found that \textbf{in certain instances, \diffcoder generated highly detailed summaries}, such summaries might not be well-suited to their requirements, leading them to prefer crafting their own summaries: \textit{"One is that its summary will be very detailed, and in this case, I might not use its result, but I would try to summarize [the summary] myself."} 
This caused them to question AI's precision and appropriateness for high-level analysis, especially in the context of oral interviews or focus groups. 


In addition, when adding codes, our participants indicated that they preferred \textbf{reading the raw data first before looking at the suggestions}, as they believed that reading the suggestions first could influence their thinking process (P1, P3, P4, P14) and introduce bias into their coding: \textit{"So I read the text at first. it makes more sense, because like, if you were to solely base your coding on [the AI agent], sometimes its suggestions and my interpretation are different. So it might be a bit off, whereas if you were to read the text, you get the full idea as to what the review is actually talking about. The suggestion functions as a confirmation of my understanding."} (P4)


\paragraph{KF3: Pre-defined data units, documented decision-making mechanisms, and progress bar features collectively enhance mutual understanding.}
\label{sec:results:KF3}

Regarding collaboration, users found that having a pre-defined unit of analysis enabled them to more easily understand the context: \textit{"I am able to see your quotations. Basically what they coded is just the entire unit. But you see if they were to code the reviews based on sentences, I wouldn't actually do the hard work based on which sentence he highlighted. But for \diffcoder, I am able to see at a glance, the exact quotations that they did. So it gives me a better sense of how their codes came about."} (P3) 
Moreover, users emphasized the importance of not only having the quotation but also keeping its context using pre-defined data units, as they often preferred to refer back to the original text. This is because understanding the context is crucial for accurate data interpretation and discussion: \textit{"I guess, it is because like we're used to reading a full text and we know like the context rather than if we were to read like short extracts from the text. the context is not fully there from just one or two line [quotations]."} (P9)


Users also appreciated \diffcoder's keywords-support function, as it \textbf{aided them in capturing finer details (P9)} and facilitated a deeper understanding of the codes added: \textit{"It presents a clearer view about that paragraph. And then it helps us to get a better idea of what the actual correct code should be. But since the other one [Atlas.ti Web] is [...] a little bit more like superficial, because it's based solely on two descriptive words."} (P14)

The progress bar feature in \diffcoder was seen as helpful when collaborating with others. It allowed them to \textbf{manage their time better and track the progress of each coder.} \textit{"I actually like the progress bar because like that I know where my collaborators are."} (P8) Additionally, it acted as a \textbf{tracker to notify the user if they missed out on a part}, which can help to avoid errors and improve the quality of coding. \textit{"So if say, for example, I missed out one of the codes then or say his percentage is at 95\% or something like that, then we will know that we missed out some parts"} (P3)


All the above features collectively improve the mutual understanding between coders, which can decrease the effort devoted to revisiting the original data and recalling their decision-making processes, and deepen discussions in limited time.


\paragraph{KF4: The shared workspace with metrics allows coders to understand disagreements and initiate discussions better.}
\label{sec:results:KF4}


In terms of statistics during the collaboration, the similarity calculation and ranking features enable users to \textbf{quickly identify (dis)agreements (P2, P3, P7, P10, P14) to ensure they focus more (P4).} As P14 said, \textit{"I think it's definitely a good thing [to calculate similarity]. From there, I think we can decide whether it's really a disagreement on whether it's actually two different information captured in the two different codes."}
Moreover, the identification of disagreements is reported to \textbf{pave the way for discussion (P1, P8)}: \textit{"So I think in that sense, it just opens up the door for the discussion compared to Atlas.ti...[and]better in idea generation stands and opening up the door for discussion."} (P8) In contrast, Atlas.ti necessitated more discussion initiation on the part of users. 

Nevertheless, ranking similarity using \diffcoder might have a negative effect, as it may make coders focus more on improving their agreements instead of providing a more comprehensive data interpretation: \textit{"I think pros and cons. because you will feel like there's a need to get high similarity on every code, but it might just be different codes. So there might be a misinterpretation."} (P7)


The participants had mixed opinions regarding the usefulness of IRR in the coding process. P9 found Cohen's kappa useful for their report as they do not need to calculate manually: \textit{"I think it's good to have Cohen’s Kappa, because we don't have to manually calculate it, and it is very important for our report. "} However, P6 did not consider the statistics to be crucial in their personal research as they usually do coding for interview transcripts. \textit{"Honestly, it doesn't really matter to me because in my own personal research, we don't really calculate. Even if we have disagreements, we just solve it out. So I can't comment on whether the statistics are relevant, right from my own personal experience."} (P6)


\paragraph{KF5: \diffcoder facilitates a top-down approach to generate code groups, which decreases the cognitive burden.}
\label{sec:results:KF5}

Participants expressed a preference for the automatic grouping function of \diffcoder, as it was \textbf{more efficient (P1, P2, P8, P14) and less labor-intensive (P3)}, compared to the more manual approach in Atlas.ti Web. 

In particular, P14 characterized the primary distinction between the two platforms as Atlas.ti Web adopts a "bottom-up approach" while \textbf{\diffcoder employs a "top-down approach".} This difference impacts the mental effort required to create categories and organize codes, as it creates "overall categories" first, allowing users to edit and shift things from a primary version instead of from scratch. \textit{"I think it's different also because  Atlas.ti is more like a bottom-top approach. So we need to see through the primary codes to create the larger categories which might be a bit more tedious, because usually, they are the primary codes. So it's very hard to see an overview of everything at once. So it takes a lot of mental effort, but for \diffcoder, it is like a top-down approach. So they [AI] create the overall categories. And then from there, you can edit and then like shift things around which helps a lot. So I also prefer \diffcoder."} (P14) P1 also highlighted this is particularly helpful when dealing with large amounts of codes, as manually grouping them one-by-one becomes nearly unfeasible.


\added{\textbf{RQ3. How can the design of CollabCoder be improved?}}

\paragraph{Attitudes towards other functions like labeling certainty, relevant codes suggestions, and individual codebook}
\label{sec:results:attitudes}


Most participants expressed concerns about the clarity, usefulness, and importance of the certainty function in \diffcoder. The self-reported nature, the potential of inconsistencies in reporting, and minimal usage among users suggest that the \textbf{certainty function may not be as helpful as intended}. For example, P12 found the certainty function "not really helpful", and P13 admitted forgetting about it due to the numerous other subtasks in the coding process. P3 also reported limited usage of the function, mainly assigning low certainty scores when not understanding the raw data. However, P14 recognized that the certainty function could be helpful in larger teams, as it might help flag quotes that require more discussion. 

The perceived usefulness of the function of the relevant code in \diffcoder depends on the dataset and users' preferences. Some participants found it \textbf{less relevant than the AI agent's summary function}, which they considered more accurate and relevant. \textit{"Maybe not that useful, but I think it depends on your dataset. Say whether they are many similar data points or whether they are different data points. So I think in terms of these cases they are all very different, have a lot of different contents. So it's not very relevant, but definitely, I think, in datasets which might be more relevant, could be useful."} (P2)


As for the individual codebook function, although users acknowledged its potential usefulness in tracking progress and handling large datasets, most users \textit{"did not pay much attention to it during this coding process"} (P2, P3, P4). 
P3 found it helpful for tracking progress but did not pay attention to it during this particular process. P4 acknowledged that the function could be useful in the long run, particularly when dealing with a large amount of data. Further exploration of these functions and their necessity may improve users' experiences with \diffcoder. 



\subsubsection{Key Findings (KF) on Collaboration Behaviors}
\paragraph{KF6: How \diffcoder workflow works under three different group dynamics}
\label{sec:results:KF6}

During the experiment, we observed various intriguing collaboration dynamics, such as \textit{"amicable cooperation"} (P3$\times$P4, P7$\times$P8, P9$\times$P10, P13$\times$P14, P15$\times$P16), \textit{"follower-leader"} (P1$\times$P2, P5$\times$P6) and \textit{"swift but less cautious"} (P11$\times$P12).

For \textit{"amicable cooperation"}, the coders respected each other's opinions. When they make a decision, they firstly identify the common keywords between their codes, and then check the suggestions with similar keywords to decide whether to use suggestions or propose their own final code decision. Often, they took turns to apply the final code. 
For example, for the first data unit, one coder might say, \textit{"hey, mine seems better, let's use mine as the final decision,"} and for the second one, the coder might say, \textit{"hey, I like yours, we should choose yours [as the final decision]"} (P3$\times$P4). In some cases, such as P13$\times$P14, both coders generally reach a consensus, displaying no strong dominance and showing respect for each other's opinions, sometimes it is challenging to finalize a terminology for the code decision. Under this kind of condition, the coders used an LLMs agent as a mediator to find a more suitable expression that takes into account both viewpoints. 

The \textit{"follower-leader"} pattern typically occurred when one coder was a novice, while the other had more expertise. Often, the inexperienced coder contributed fewer ideas or only offered support during the coding process: when using Atlas.ti Web, those "lead" coders tended to take on more coding tasks than the others since their coding tasks could not be precisely quantified. Even though both of them were told to code all the data, it would end up in a situation where one coder primarily handled the work and the other merely followed with minimal input. This pattern could also appear if the coders worked at different paces (P1$\times$P2). As a result, the more efficient coders expressed more ideas. In contrast, \diffcoder ensures equitable participation by assigning the same coding workload to each participant and offering detailed documentation of the decision-making process via its independent coding interface. This approach guarantees that coders, even if they seldom voice their opinions directly, can still use the explicit documented information to communicate their ideas indirectly and be assessed in tandem with their collaborators. Furthermore, the suggestions generated by GPT are derived from both codes and raw data, producing a similar effect.

The \textit{"swift but less cautious"} collaboration was a less desirable pattern we noticed: For P11$\times$P12, during the merging process, they would heavily rely on GPT-generated decisions in order to finish the task quickly. This scenario highlights the concerns regarding excessive reliance on GPT and insufficient deep thinking, which can negatively impact the final quality even when GPT is used as a mediator after the codes have been produced, as defined as our initial objective. Under this pattern, the pair sadly used GPT for "another round of coding" rather than as a neutral third-party decision advice provider.






% Gao et al.\cite{gao2023coaicoder} underscore the challenges of maintaining coding independence, often sacrificed for efficiency in real-world scenarios. \diffcoder counters this by enabling users to smoothly navigate the CQA process while preserving coding independence, thereby achieving our initial design goals (\hyperref[sec:design_goal_1]{DG1} and \hyperref[sec:design_goal_2]{DG2}). \hyperref[sec:design_goal_4]{DG4}, is also achieved by \hyperref[sec:results:KF3]{KF3}: users found that pre-defined code units helped them grasp the context of the codes, facilitating the building of mutual understanding.  \hyperref[sec:design_goal_5]{DG5} will be addressed later in Section \ref{sec:disc:llm_suggestion_provider}. Additionally, \diffcoder fosters enhanced mutual understanding among users by creating a shared space for transparent communication \footnote{\url{https://workplace.msu.edu/transparent-communication/\#:~:text=At\%20a\%20Glance-,Transparent\%20communication\%20is\%20the\%20act\%20of\%20both\%20good\%20and\%20bad,Increases\%20collaboration}}, significantly improving collaboration and decision-making, thus meeting further design goals (\hyperref[sec:design_goal_6]{DG6} and \hyperref[sec:design_goal_7]{DG7}). 
% Our approach also facilitates identifying (dis)agreements through similarity scores, streamlining discussions to focus on critical debates, leading to more thorough discussions and higher IRRs (see Table \ref{tab:result}). However, for \hyperref[sec:design_goal_3]{DG3}, since \diffcoder incorporated a feature from Atlas.ti Web, the results do not provide a straight assessment. Future research could explore if using a web-based and centralized design might improve users' efficacy in collaborative tasks, which is a limitation of our current study.

